How to Train Your CheXDragon: Training Chest X-Ray Models for Transfer to Novel Tasks and Healthcare Systems

Self-supervised learning (SSL) enables label efficient training for machine learning models. This is essential for domains such as medical imaging, where labels are costly and time-consuming to curate. However, the most effective supervised or SSL strategy for transferring models to different healthcare systems or novel tasks is not well understood. In this work, we systematically experiment with a variety of supervised and self-supervised pretraining strategies using multimodal datasets of medical images (chest X-rays) and text (radiology reports). We then evaluate their performance on data from two external institutions with diverse sets of tasks. In addition, we experiment with different transfer learning strategies to effectively adapt these pretrained models to new tasks and healthcare systems. Our empirical results suggest that multimodal SSL gives substantial gains over unimodal SSL in performance across new healthcare systems and tasks, comparable to models pretrained with full supervision. We demonstrate additional performance gains with models further adapted to the new dataset and task, using multimodal domain-adaptive pretraining (DAPT), linear probing then finetuning (LP-FT), and both methods combined. We offer suggestions for alternative models to use in scenarios where not all of these additions are feasible. Our results provide guidance for improving the generalization of medical image interpretation models to new healthcare systems and novel tasks.

==> templates/datasets.tex <==
% \section{Datasets}

% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \textbf{Dataset}                        & \textbf{\# Train} & \textbf{\# Val} & \textbf{\# Test} & \textbf{\# Total} \\ \hline
% \textbf{CheXpert}                       & 218,414           & 5,000           & 1,000            & 224,414           \\ \hline
% \textit{Atelectasis}                    & 65,634            & 1,481           & 200              & 67315             \\
% \textit{Cardiomegaly}                   & 34,290            & 797             & 200              & 35287             \\
% \textit{Consolidation}                  & 41,546            & 979             & 200              & 42725             \\
% \textit{Edema}                          & 63,798            & 1,432           & 200              & 65430             \\
% \textit{Pleural Effusion}               & 95,620            & 2,195           & 200              & 98015             \\ \hline
% \textbf{Intermountain}                  & 19,028            & 3,361           & 2,256            & 21,184            \\ \hline
% \textit{Pneumonia}                      & 12,499            & 736             & 630              & 13865             \\
% \textit{Pneumonia+Pleural Effusion}     & 1,628             & 95              & 61               & 1784              \\
% \textit{Pneumonia+Multilobar Pneumonia} & 4,390             & 376             & 419              & 5185              \\ \hline
% \textbf{CANDID-PTX}                     & 15,387            & 1,923           & 1,923            & 19,237            \\ \hline
% \textit{Pneumothorax}                   & 2,553             & 323             & 320              & 3196              \\
% \textit{Rib Fracture}                   & 254               & 41              & 40               & 335               \\
% \textit{Chest Tube}                     & 1,149             & 140             & 134              & 1423              \\ \hline
% \end{tabular}
% \vspace{0.3cm}
% \caption{Dataset statistics for CheXpert, Intermountain, and CANDID-PTX. For each dataset overall, the numbers presented indicate the total number of studies per split. Within each task, the numbers presented indicate the number of studies \textit{positive for the task} per split.}
% \label{table:data_stats}
% \end{table}

% \subsubsection{CheXpert}
% "CheXpert" is a large public dataset of 224,316 chest X-ray studies of 65,240 patients, collected from inpatients and outpatients at Stanford Health Care between 2002 and 2017. Each study has an associated radiology report (not publically available) dictated by a radiologist during clinical care. Each study is also labeled, via an automatic rules-based labeler, for 14 binary clinical observations, which we use as our pretraining tasks: No Finding, Cardiomegaly, Enlarged Cardiomegaly, Lung Lesion, Lung Opacity, Edema, Consolidation, Pneumonia, Atelectasis, Pneumothorax, Pleural Effusion, Pleural Other, Fracture, and Support Devices. The "competition", or test, tasks for CheXpert are a subset of the above: Atelectasis, Cardiomegaly, Consolidation, Edema, and Pleural Effusion.

% \subsubsection{Intermountain}
% "Intermountain" is our first external institution, or "downstream", dataset. It is a private dataset containing 21,184 chest X-ray studies, collected at outpatient centers---5 emergency departments and 22 urgent care centers that are part of the Intermountain Health network (Utah, USA) between 2009 and 2021. Like CheXpert, each study has an associated radiology report dictated by a radiologist for clinical care. Each study is also labeled by a radiologist for 3 pneumonia-related clinical observations: Pneumonia, Pleural Effusion, and Multilobar/Multifocal Pneumonia. This dataset contains labels for Pleural Effusion, and Multilobar/Multifocal Pneumonia only for patients positive for Pneumonia. We formulate these tasks as three binary classification tasks - Pneumonia only, Pneumonia and Pleural Effusion, and Pneumonia and Multilobar/Multifocal Pneumonia. 

% \subsubsection{CANDID-PTX}
% "CANDID-PTX" is our second downstream dataset. It is a public dataset containing 19,237 chest X-ray studies, collected at Dunedin Hospital (Dunedin, NZ) between 2010 and 2020. Like CheXpert, each study has an associated radiology report dictated by a radiologist for clinical care. Each study is labeled for 3 clinical observations: Pneumothorax, Acute Rib Fracture, and Intercostal Chest Tube. We format all three prediction tasks as binary classification tasks ("negative"/"positive").

==> templates/results_table.tex <==
\begin{table}
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|c|c c c c|c c c c c c|}
\hline
 \textbf{\shortstack{Labeled\\Fraction}} & 
 \textbf{\shortstack{Pretraining\\Dataset}} & \textbf{\shortstack{Pretraining\\Objective}} & 
 \textbf{\shortstack{NO-DAPT/\\DAPT?}} &
 \textbf{\shortstack{LP/\\LP-FT?}} &
 \textbf{\shortstack{Macro-\\AUROC}} &  \textbf{\shortstack{Micro-\\AUROC}} & \textbf{\shortstack{Macro-\\AUPRC}} & \textbf{\shortstack{Micro-\\AUPRC}} & \textbf{\shortstack{Macro-\\F1}} &  \textbf{\shortstack{Micro-\\F1}} \\
\hline
\multirow{12}{*}{0.01}  
&  ImageNet & Sup & NO-DAPT & LP & 0.548 & 0.721 & 0.152 & 0.234 & 0.073 & 0.187 \\
&  ImageNet & Sup & DAPT & LP & 0.705 & 0.781 &  0.34 & 0.462 & 0.206 & 0.338 \\
&  ImageNet & Sup & NO-DAPT & LP-FT & 0.587 & 0.536 & 0.177 & 0.182 &0.2 & 0.246 \\
&  ImageNet & Sup & DAPT & LP-FT &  0.86 & 0.906 & 0.489 & 0.651 & 0.388 & 0.594 \\
\hdashline
&  CheXpert & Sup & NO-DAPT & LP & 0.812 &  0.85 & 0.423 & 0.567 & 0.168 &  0.386 \\
&  CheXpert & Sup & DAPT & LP &  0.77 & 0.855 & 0.456 & 0.601 & 0.171 & 0.375 \\
&  CheXpert & Sup & NO-DAPT & LP-FT &  \underline{0.87} & 0.896 & 0.503 & 0.647 & 0.315 &  0.562 \\
&  CheXpert & Sup & DAPT & LP-FT & 0.866 & \underline{0.911} &  \underline{0.55} & \underline{0.701} & \underline{0.396} & \underline{0.632} \\
\hdashline
&  CheXpert & GLoRIA & NO-DAPT & LP & 0.672 & 0.804 & 0.327 & 0.477 & 0.096 & 0.234 \\
&  CheXpert & GLoRIA & DAPT & LP & 0.817 & 0.888 & 0.492 & 0.656 & 0.232 & 0.476 \\
&  CheXpert & GLoRIA & NO-DAPT & LP-FT & 0.837 & 0.876 & 0.461 & 0.601 & 0.278 & 0.513 \\
&  CheXpert & GLoRIA & DAPT & LP-FT & \textbf{0.874} &  \textbf{0.92*} & \textbf{0.555*} & \textbf{0.718*} & \textbf{0.416} & \textbf{0.649*} \\
\hline
\multirow{12}{*}{0.1}  
&  ImageNet & Sup & NO-DAPT & LP & 0.709 & 0.795 & 0.273 & 0.352 & 0.102 & 0.228 \\
&  ImageNet & Sup & DAPT & LP &0.9 & 0.931 & 0.556 & 0.725 & 0.471 & 0.663 \\
&  ImageNet & Sup & NO-DAPT & LP-FT & 0.821 & 0.854 & 0.417 & 0.545 & 0.377 & 0.538 \\
&  ImageNet & Sup & DAPT & LP-FT & 0.901 & 0.934 & 0.575 & 0.735 & 0.519 & 0.679 \\
\hdashline
&  CheXpert & Sup & NO-DAPT & LP & 0.907 & 0.925 &  0.59 & 0.721 & 0.491 & 0.653 \\
&  CheXpert & Sup & DAPT & LP & 0.921 & 0.945 & 0.635 & 0.787 & 0.556 & 0.718 \\
&  CheXpert & Sup & NO-DAPT & LP-FT & 0.919 & 0.938 & 0.638 & 0.763 & 0.567 & 0.704 \\
&  CheXpert & Sup & DAPT & LP-FT & 0.925 & 0.947 & \underline{0.648} & \underline{0.796} & \underline{0.575} & \underline{0.727} \\
\hdashline
&  CheXpert & GLoRIA & NO-DAPT & LP & 0.9 & 0.922 & 0.579 & 0.713 & 0.469 & 0.641 \\
&CheXpert & GLoRIA & DAPT & LP & \underline{0.926} & \underline{0.948} & 0.629 &  0.79 & 0.555 &  0.72 \\
&  CheXpert & GLoRIA & NO-DAPT & LP-FT & 0.908 & 0.935 &  0.62 &  0.76 & 0.545 & 0.697 \\
&  CheXpert & GLoRIA & DAPT & LP-FT &  \textbf{0.93} & \textbf{0.949} & \textbf{0.651} & \textbf{0.798} & \textbf{0.577} & \textbf{0.728} \\
\hline
\multirow{12}{*}{1}  
&  ImageNet & Sup & NO-DAPT & LP & 0.815 & 0.852 & 0.398 &  0.47 & 0.275 & 0.419 \\
&  ImageNet & Sup & DAPT & LP & 0.914 & 0.938 & 0.597 & 0.746 & 0.513 & 0.682 \\
&  ImageNet & Sup & NO-DAPT & LP-FT & 0.908 & 0.927 & 0.609 & 0.735 & 0.546 & 0.693 \\
&  ImageNet & Sup & DAPT & LP-FT & 0.923 & 0.942 & 0.651 & 0.773 & 0.617 & 0.719 \\
\hdashline
&  CheXpert & Sup & NO-DAPT & LP & 0.926 & 0.939 & 0.649 & 0.764 & 0.554 & 0.689 \\
&  CheXpert & Sup & DAPT & LP & 0.936 & \underline{0.952} & 0.665 & 0.806 & 0.586 & 0.731 \\
&  CheXpert & Sup & NO-DAPT & LP-FT & 0.937 &  0.95 & \textbf{0.703*} & 0.803 & 0.655 & 0.748 \\
&  CheXpert & Sup & DAPT & LP-FT & 0.936 & \underline{0.952} & \underline{0.7} & \underline{0.816} & \textbf{0.662} & \underline{0.758} \\
&  CheXpert & GLoRIA & NO-DAPT & LP & 0.921 & 0.934 & 0.627 & 0.746 & 0.545 & 0.677 \\
&  CheXpert & GLoRIA & DAPT & LP & \underline{0.938} & \underline{0.952} &  0.66 & 0.805 & 0.585 & 0.728 \\
&  CheXpert & GLoRIA & NO-DAPT & LP-FT & 0.932 & 0.945 & 0.661 & 0.775 & 0.627 & 0.732 \\
&  CheXpert & GLoRIA & DAPT & LP-FT & \textbf{0.946} & \textbf{0.955} & \textbf{0.703*} & \textbf{0.822} & \underline{0.659} & \textbf{0.759} \\
\hline
\end{tabular}
}
 \vspace{0.2cm}
 \caption{
     Results for ImageNet & Supervised, CheXpert & Supervised, and CheXpert & GLoRIA models at label fractions of 0.01, 0.1, and 1. For each initial pretrained model type, we show results with a simple linear probe ("+LP"), with linear probing, then finetuning ("+LP-FT"), with domain-adaptive pretraining and a linear probe ("+DAPT+LP"), and with domain-adaptive pretraining and linear probing, then finetuning ("+DAPT+LP-FT"). Best result within each label fraction is \textbf{bolded} and next-best is \underline{underlined}. There are no statistically significant difference between the best model result over the next-best model result (95\% CI), so we denote a statistically significant difference between the best model result and the third-best with "*".
 }
 \label{table:results}
\end{table}

